A flexured-gimbal 3-axis force-torque sensor reveals minimal cross-axis coupling in an insect-sized flapping-wing robot

The mechanical complexity of flapping wings, their unsteady aerodynamic flow, and challenge of making measurements at the scale of a sub-gram flapping-wing flying insect robot (FIR) make its behavior hard to predict. Knowing the precise mapping from voltage input to torque output, however, can be used to improve their mechanical and flight controller design. To address this challenge, we created a sensitive force-torque sensor based on a flexured gimbal that only requires a standard motion capture system or accelerometer for readout. Our device precisely and accurately measures pitch and roll torques simultaneously, as well as thrust, on a tethered flapping-wing FIR in response to changing voltage input signals. With it, we were able to measure cross-axis coupling of both torque and thrust input commands on a 180 mg FIR, the UW Robofly. We validated these measurements using free-flight experiments. Our results showed that roll and pitch have maximum cross-axis coupling errors of 8.58% and 17.24%, respectively, relative to the range of torque that is possible. Similarly, varying the pitch and roll commands resulted in up to a 5.78% deviation from the commanded thrust, across the entire commanded torque range. Our system, the first to measure two torque axes simultaneously, shows that torque commands have a negligible cross-axis coupling on both torque and thrust.

==> extra.tex <==
\begin{comment}

\section{Dynamic Analysis and Torque Generation in Trimming}

\subsection{Dynamic Analysis of trimming}


\begin{figure}[t] 
      \centering
      \includegraphics[width= 2.8 in]{images/dynamic_model_YC.png}
      \caption{Dynamic model of the fly used for calculating pitch and roll trims. Here $O_x$ and $O_y$ are centers roll and pitch flexures respectively.}
      \label{dynamics_robofly}
\end{figure}


The attitude dynamics of a generic 6 dof rigid body evolve in time according to the equation.
\begin{equation}
\dot\theta= \mathbf{W}(\theta)\omega
\label{eom1}
\end{equation}
\begin{equation}
\mathbb{J}\dot\omega= \tau- \omega \times \mathbb{J}\omega
\label{eom2}
\end{equation}
where $\theta\in \mathbb{R}^3$ is the attitude of the robot, defined by three Euler Angles. Here Euler Angles are used to describe the motion in the neighbourhood of certain attitude so the fact that they have singularities at extreme attitudes can be ignored. The Euler Angles are given in zyx-order: the attitude is obtained by first rotating an angle $\theta_z(yaw)$ around the body z-axis, then by $\theta_y(pitch)$ around the new body y-axis, and then $\theta_x(roll)$ around the new body x-axis. The rest of the quantities are all in body-frame coordinates: $\mathbb{J}\in \mathbb{R}^{3X3}$ is the matrix of the moment of inertia, $\omega \in \mathbb{R}^3$ is the angular velocity vector of the robot, and $\tau \in \mathbb{R}^3$ is the sum of all torques or moments applied to the body, primarily aerodynamic forces and control torques.  The quantity $\mathbf{W}(\theta)\in \mathbb{R}^{3\times3}$ is a matrix that relates the angular velocity $\omega$ to the rate of change in Euler Angles in Equation (1) and can be rewritten in terms of body coordinates to give
 \begin{equation}
  \left[ {\begin{array}{c}
   \dot\theta_x\\
   \dot\theta_y\\
   \dot\theta_z\\
  \end{array} } \right]=
  \left[ {\begin{array}{c c c}
   1 & \sin\theta_x \tan\theta_y &\cos\theta_x \tan\theta_y\\
   0 & \cos\theta_x  & -\sin\theta_x \\
   0 & \sin\theta_x /\cos\theta_y & \cos\theta_x/ \cos\theta_y\\
  \end{array} } \right]
  \left[ {\begin{array}{c}
   \omega_1\\
   \omega_2\\
   \omega_3\\
  \end{array} } \right]
 \end{equation}
 
 Either on board IMU or motion capture system can be used to get an estimate of attitude, parameterized by $\theta$. These measurement with Eq.~\ref{eom1} and Eq.~\ref{eom2} can be used to estimate the bias torque $\tau_b$ on the robot in a short flight, given by
 \begin{equation}
     \hat\omega= \mathbf{W}^{-1}(\theta) \dot{\theta}
 \end{equation}
 \begin{equation}
     \hat\tau_b= \mathbb{J}(\Hat{\dot{\omega}}) + \hat\omega \times \mathbb{J}\hat\omega
     \label{bias_eom}
 \end{equation}
Here an assumption is made that all torques such as from aerodynamic drag and gyroscopic effects are negligible. This assumption holds if the robots velocity remains small. The setup for the trim calculation is made in such a way that the robot is only allowed to move in pitch and roll. So, we can assume that $\omega_3$ is zero. To make the math simpler we assume inertia matrix is diagonal, $\mathbb{J}= diag(J_1,J_2,J_3)$, thus making the term $\omega \times \mathbb{J}\omega \approx 0$. Consequently, Eq. \ref{bias_eom} is reduced to 
\begin{equation}
    \Hat{\tau_b}= \mathbb{J}\Hat{\dot{\omega}}
    \label{tau_bias_omega}
\end{equation}
\end{comment}
\begin{comment}
\subsection{Amplitude Frequency Experiments} 
\textcolor{magenta}
{Several experiments are done with the fly at different amplitudes and frequencies. These experiments are important to find the resonance frequency of the wings as the wings generates maximum thrust at resonance. For characterization of the new design the frequency experiments are performed at different amplitudes. This characterization helped us in learning the relation between the Amplitude and thrust of this new design. Robofly expanded is  held on a carbon-fiber rod at-least 15 cm above the ground to avoid any ground effect. The whole setup is placed on a scale to measure the thrust.  These values are plotted 
}


\subsection{Trimming on Quadrotor}

As trimming is an important step for a stable controller, most of the commercially available quad rotors have provisions for manual setting of roll and pitch trim. However, sometimes you can still achieve a good flight without giving any trim due to comparatively slower and more stable dynamics of a quad. Crazyflie was mounted on the quad rotor trimming device (Fig. \ref{Photo_crazyflie}) and equal weights were hanged from each side of the flexures to bring centre of mass down and make the system more stable.

State feedback obtained form the IMU  at the frequency of 100Hz is fed to an integral controller which estimated the bias values between -1 to 1. These values are then mapped to the motor speeds of the quad, the sign of the bias value will signify which motor to reduce speed on the value will define the percentage. The bias values map to the corresponding motor thrust percentage as $m1=100\%, m2=85\%, m3=100\%, m4=95\%$. The output of the controller and the corresponding roll and pitch angles can be seen in Fig. ~\ref{Graph_crazyflie}. The analysis is done for a 10 seconds window in which the pitch and roll angles slowly come to 0.
  \begin{figure}[t] 
      \centering
      \includegraphics[width= 3.5 in]{images/graph_quad.eps}
      \caption{ }
      \label{Graph_crazyflie}
   \end{figure}

\begin{figure}[ht] 
      \centering
      \includegraphics[width= 3.5 in]{images/without_control.eps}
      \caption{Pitch and Roll angles in an open loop 12 seconds flight of a  RoboFly while mounted on the trimming device.}
      \label{without_control}
   \end{figure}


\begin{figure}[ht] 
      \centering
      \includegraphics[width= 3.5 in]{images/Robo_fly_controlled.eps}
      \caption{The grap}
      \label{Graph_robofly}
   \end{figure}
\end{comment}
\begin{comment}
\subsection{Trimming Device for quad rotor}
We used Crazyflie, a commercially available open source quad rotor, for the proof of concept here. Crazyflie is mounted on a set of two flexure joints as shown in ~\ref{Photo_crazyflie}, limiting its unconstrained degrees of freedom to two, pitch and roll. We chose flexures instead of pin joints because the same concept will be applied to the RoboFly and we wanted the setup to be similar.The flexures we used are made from thin polystyrene sheet sandwiched between two 1.5mm card-boards. The two flexures are held together by joining plate made from same material with grooves perpendicular to each other on either side. Crazyflie is mounted on the setup using two  3 mm screws.
  \begin{figure}[t] 
      \centering
      \includegraphics[width= 2.5 in]{images/quad_on_flex.png}
      \caption{The figure shows the experimental setup for the quad rotor to calculate the pitch and roll torque biases}
      \label{Photo_crazyflie}
   \end{figure}
\end{comment}

\subsection{Gains in trimming\textcolor{cyan}{Yogesh's subsection, work in eqs for pi control and rotational dynamics with ontrol and restoring torque from mass or flexure probably go here}}


   
 The position and orientation of the robot when fixed on trimming device are shown in Fig. \ref{kinematics}. The roll and pitch joints, J1 and J2 respectively, are designed to support the roll and pitch motion in the body frames of the robot. The (X,Y,Z) represents the world coordinate system, whereas (X1,Y1,Z1) and (X2,Y2,Z2) represent the the coordinate systems attached with links L1 and L2, respectively. Therefore, (X2,Y2,Z2) are nothing but the body coordinate system of the robot.
 
 These joints have minimal drag torque about their respective rotational axes. The drag torque is directly proportional to the stiffness of the hinge as given in Eq. \ref{stiffness_equation}. However, the stiffness is significantly larger about other axes than its angle of rotation. We will now consider two extreme cases to demonstrate the role of gains in trimming and which of the rotational motions should be corrected as a top priority. First extreme case of a large roll bias of 90$^\circ$, we can imagine that Y1 will coincide with -Z axis. If robot has to perform a small pitch motion $\theta_p$, it will take place about the body-Y axis, which is Y2. Since the joint J2 is free to move about Y2 axis, the robot can perform both of its rotational motions in case of extreme roll bias. Now, considering the second extreme case of a large pitch bias of 90$^\circ$, we can imagine X2 coinciding with -Z1. If the robot is to perform roll by a small angle $\theta_r$, it needs to happen about -Z1 axis of the joint J1, which is practically impossible, since J1 is supposed to rotate freely only about X1 axis. Therefore, to accurately determine the roll bias, pitch gain is set to a larger value to achieve a nearly constant pitch first.
 
 Another possible case is to rotate the robot about its yaw axis by 90$^\circ$ while fixing on the device. In this case, the joints J1 and J2 would switch the roles to become the pitch and roll joints, respectively. As contrary to above case, we have to set larger gain for controlling roll motion.

\begin{figure}[t] 
      \centering
      \includegraphics[width= 2.8 in]{images/torque_change.png}
      \caption{Representation of roll offset in the mounting of the robot. Robot is attached with non-stationary end of pitch link through the connecting rod, passing though its centre of mass $(COM_R)$. \textcolor{magenta}{Yogesh: I can barely see your axes}}
      \label{COM_imbalance}
\end{figure}
  \begin{figure}[t] 
      \centering
      \includegraphics[width= 2.5 in]{images/kinematics.png}
      \caption{ Schematic of the flexure device designed in this work. There are two flexure joints, J1 and J2 to support roll and pitch motions of the robot, respectively.}
      \label{kinematics}
   \end{figure}





Justify torque target accuracy later: torques that are typically induced by the wire tether~\cite{fuller2014controlling}. Given that the wire tether represents an unpredictable torque that is random and time-varying, the target precision of our torque bias estimation device is therefore to trim the system to within that torque. Therefore, the error introduced by a small $O_R$ is much larger than our desired error bound, and must therefore be eliminated. 

==> extra_2.tex <==

\section{Design and Fabrication of Trimming Device}

 \begin{figure*}[t]
      \centering
      \includegraphics[width=7in]{images/combined.png}
      \caption{(a) The roll link of the trimming device. The link is folded around the castellated joint so the fly can be held perpendicular to the roll flexure and parallel to the ground. (b) The pitch link of the device. Its attached to the roll link via  protrusions on top. c) The whole assembly of trimming device, the fly is attached to the pitch link on the bottom. \textcolor{cyan}{make them of same scale}}
      \label{felx_1}
   \end{figure*}

\subsection{Design Considerations}

The trimming device has two links roll link \textcolor{magenta}{Fig.~\ref{felx_1}~(a) and pitch link Fig~\ref{felx_1}~(b)}. Each link has a stationary part and a non-stationary part. The stationary part of roll link is attached to the ground and the stationary part of the pitch link is attached to the non-stationary part of the roll link. The robot would be mounted on the non-stationary part of pitch link through the connecting rod.  Roll link has a slot cut in the centre to allow the pitching of the robot. These links are separated by a minimum distance on the vertical axis so as to avoid any large moments. The roll link is just 15~mm in width to preclude any ground effect.

A small 10~mm $\times$ 15~mm aligning plate is mounted on the top of the connecting rod. To facilitate the alignment of robot's centre of mass with the axis of flexure as explained in section III (B).

\subsection{Fabrication of the trimming Device}
The links are made up of 12~$\mu$ Kapton sandwiched between layers of 254~$\mu$ FR4. Bending stiffness of the flexure joint, $K_{stiff}$ was calculated by using $K_{stiff}= \frac{Et^3w}{12L}$ \cite{malka2014principles}. Here, $t$ is thickness of the flexure material, $L$ is length of the flexure joint which is kept at 500~$\mu$, $w$ is width of the joint which is 3~mm and E is the Young's modulus of 2.5~Gpa. These parameters are carefully selected to keep the stiffness of the joint at really low value of 2.16~$\times \mu$ Nm.\textcolor{magenta}{it would be great to add here a prediction of the angle produced by a 1~$\mu$Nm torque, which is about the max that robots of this scale can produce (cite ma2012, which measured it} Here, the minimum flexure bending stiffness ensures faster convergence to the steady state trim values. 

For the roll link, flexure and castellated cuts were made on the top and bottom FR4 layers. Similar features are cut out on the pyralux adhesive layer. This link is designed to be folded along the axis of castellated joint. For the pitch link only flexure cut was made on top and bottom FR4 layers, and similar features are cut on pyralux adhesive layers. The layers were laminated together in a heat press under a force of $50 Kg$. A release cut was done afterwards to extract the required links from its scaffolding.  The assembly of the device can be seen in Fig.~\ref{felx_1}~(c) where the two links are glued together. The outer boundary of the roll link is connected to a 




These torque generation techniques are used to determine the bias torques when the robot is fixed on the trimming device. Eq.~\ref{torque_equation} can be re-written for roll and pitch about the roll flexure axis $O_x$ and pitch flexure axis $O_y$ respectively  (Fig.~\ref{cartoon:dynamics_robofly}) as Eq.~\ref{tau_bias_omega_eom}.
\begin{align}
\begin{aligned}
    J_{roll}\ddot{\theta}_x = (T_1- T_2) b- m_Rgp+ m_bgq - k_{stiff}\theta_x\\
    J_{pitch}\ddot{\theta}_y = -(T_1+T_2) d+ m_Rgr -m_bgs -k_{stiff}\theta_y
\end{aligned}\label{tau_bias_omega_eom}
\end{align}




Here $m_R$ is the mass of the robot, $k_{stiff}$ is the flexure stiffness, which is same for both roll and pitch joints, and $m_b$ is the mass of the balancing weight, used to decrease the height of the centre of mass of the system. In front view, b is the distance between the center of mass of the robot $(COM_R)$ and the aerodynamic center (AC) of the wings, $p$ is the horizontal distance between roll flexure joint and $COM_R$, $q$ is the horizontal distance between the centre of balancing weight and the roll flexure joint, in side view, $d$ is the distance between AC and  $COM_R$, $r$ is the horizontal distance between $COM_R$ and the pitch flexure joint and $s$ is the horizontal distance between centre of balancing weight and the pitch flexure joint,

To calculate the bias torque an integral controller is used represented in Eq.~\ref{controller_equation}. 
\begin{align}
\begin{aligned}
     J_{roll}\ddot{\theta}_x&= (T_1-T_2) b- m_Rgp+ m_bgq - k_{stiff}\theta_x - K_i^{roll}\int_{\theta_x}^{0}\theta d\theta\\
     J_{pitch}\ddot{\theta}_y&= -(T_1+T_2) d+ m_Rgr -m_bgs -k_{stiff}\theta_y + K_i^{pitch}\int_{\theta_y}^{0}\theta d\theta
\end{aligned}\label{controller_equation}
\end{align}
Here, $K_i^{roll}$ and $K_i^{pitch}$ are integral controller gains for roll and pitch respectively. At the steady state, the terms $\theta_x$ ,$\theta_y$,$\ddot{\theta}_x$, $\ddot{\theta}_y$,$p$,$q$,$r$ and $s$ would be zero and the integral term in Eq.~\ref{controller_equation} would give the required bias torques.


